FEDformer: Frequency Enhanced Decomposed Transformer for Long-term Series Forecasting

Although Transformer-based methods have significantly improved state-of-the-art results for long-term series forecasting, they are not only computationally expensive but more importantly, are unable to capture the global view of time series (e.g. overall trend). To address these problems, we propose to combine Transformer with the seasonal-trend decomposition method, in which the decomposition method captures the global profile of time series while Transformers capture more detailed structures. To further enhance the performance of Transformer for long-term prediction, we exploit the fact that most time series tend to have a sparse representation in well-known basis such as Fourier transform, and develop a frequency enhanced Transformer. Besides being more effective, the proposed method, termed as Frequency Enhanced Decomposed Transformer ({\bf FEDformer}), is more efficient than standard Transformer with a linear complexity to the sequence length. Our empirical studies with six benchmark datasets show that compared with state-of-the-art methods, FEDformer can reduce prediction error by $14.8\%$ and $22.6\%$ for multivariate and univariate time series, respectively. Code is publicly available at https://github.com/MAZiqing/FEDformer.

==> tables/tab_ablation_about_QKVR.tex <==

\begin{table*}[t]
% \begin{adjustwidth}{-1.5in}{-1in}
\begin{tabular}{c|c|cccccccccccccc}
\toprule
\multicolumn{2}{c|}{Methods}&\multicolumn{2}{c|}{Autoformer}&\multicolumn{2}{c|}{Fedformer v1}&\multicolumn{2}{c|}{Fedformer v2}&\multicolumn{2}{c|}{Fedformer-f}&\multicolumn{2}{c|}{Fedformer+R}&\multicolumn{2}{c|}{R(self+cross)}&\\
\midrule

\multirow{2}{*}{Detail} 
% & 48 & 0.454 & & 0.366 & & 0.476 & & 0.356 \\
& Self-att & \multicolumn{2}{c|}{AutoCorrelation} & \multicolumn{2}{c|}{FNO (Eq. \ref{func:FNO-self})} & \multicolumn{2}{c|}{AutoCorrelation} & \multicolumn{2}{c|}{FNO (Eq. \ref{func:FNO-self})}& \multicolumn{2}{c|}{Q.R}& \multicolumn{2}{c|}{Q.Q.Q.R}\\
& Corss-att & \multicolumn{2}{c|}{AutoCorrelation} & \multicolumn{2}{c|}{AutoCorrelation} & \multicolumn{2}{c|}{FNO (Eq. \ref{func:FNO-Corss})} & \multicolumn{2}{c|}{FNO (Eq. \ref{func:FNO-Corss})}&\multicolumn{2}{c|}{Q.K.V.R}&\multicolumn{2}{c|}{Q.K.V.R}\\
\midrule

\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE \\%& MSE  & MAE \\
\midrule
\multirow{4}{*}{\rotatebox{90}{ETTm1}} 
% & 48 & 0.454 & & 0.366 & & 0.476 & & 0.356 \\
& 96 & 0.481 & 0.463 & \textbf{0.378} & \textbf{0.419} &  0.539 & 0.490 & \textbf{0.379} & \textbf{0.419} & 0.379 & 0.419& 0.453&0.455\\
& 192 & 0.628 & 0.526 & \textbf{0.417} & \textbf{0.442} & \textbf{0.556} & \textbf{0.499} & \textbf{0.426} & \textbf{0.441}& 0.424 & 0.441&0.475& 0.468 \\
% & 288 & 0.634 & & 0.430 & & 0.571 & & 0.379 \\
& 336 & 0.728 & 0.567 & \textbf{0.480} & \textbf{0.477} & \textbf{0.541} & \textbf{0.498} & \textbf{0.445} & \textbf{0.459} & 0.446 & 0.458 &0.492 &0.478\\
% & 672 & 0.606 & & 0.528 & & 0.544 & & 0.501\\
& 720 & 0.658 & 0.548 & \textbf{0.543} & \textbf{0.517} & \textbf{0.558} & \textbf{0.507} & \textbf{0.543} & \textbf{0.490} &0.540 &0.490 &0.520 &0.495 \\
\midrule
\multirow{4}{*}{\rotatebox{90}{ETTm2}} 
& 96 & 0.255 & 0.339 & 0.259  & \textbf{0.337}& \textbf{0.216} &\textbf{0.297} &\textbf{0.203} & \textbf{0.287}  & & & 0.211 & 0.293    \\
& 192 & 0.281 & 0.340 & 0.285 & 0.344& \textbf{0.274} &\textbf{0.331} & \textbf{0.269} & \textbf{0.328}  & & & 0.270 &0.328    \\
& 336 & 0.339 & 0.372 & \textbf{0.320} & 0.373& \textbf{0.334} &\textbf{0.369} & \textbf{0.325} & \textbf{0.366} & & & 0.325& 0.363    \\
& 720 & \textbf{0.422} & \textbf{0.419} & 0.761 & 0.628& 0.427 &0.420 & \textbf{0.421} & \textbf{0.415} & & &0.416 &0.414\\
\midrule
\multicolumn{2}{c|}{Count} & 1 & 1 & 5 & 5 & 6 & 6 & 8 & 8\\
\bottomrule
\end{tabular}
\caption{Ablation: multivariate long sequence time-series forecasting results on six datasets.}
\label{tab:ablation_R}
% \end{adjustwidth}
\end{table*}

==> tables/tab_benchmark_m.tex <==
%\resizebox{!}{\.5\paperheight}{
\begin{table*}[t]
\centering
\begin{footnotesize}
% \begin{adjustwidth}{-1.5in}{-1in}
\caption{multivariate long-term series forecasting results on six datasets with input length $I=96$ and prediction length $O \in \{96,192336,720\}$ (For ILI dataset, we use input length $I=36$ and prediction length $O \in \{24,36,48,60\}$). A lower MSE indicates better performance.}
\scalebox{0.85}{
\begin{tabular}{c|c|cccccccccccccccc}
\toprule
\multicolumn{2}{c|}{Methods}&\multicolumn{2}{c|}{FEDformer-f}&\multicolumn{2}{c|}{FEDformer-w}&\multicolumn{2}{c|}{Autoformer}&\multicolumn{2}{c|}{Informer}&\multicolumn{2}{c|}{LogTrans}&\multicolumn{2}{c}{Reformer}\\
\midrule
\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE\\
\midrule
\multirow{4}{*}{\rotatebox{90}{$ETTm2$}} &96 & \textbf{0.203} & \textbf{0.287} &0.204 &0.288 &0.255  &0.339  &0.365  &0.453  &0.768  &0.642  &0.658  &0.619    \\
                        & 192 & \textbf{0.269} & \textbf{0.328} &0.316  &0.363  &0.281 &0.340 &0.533  &0.563  &0.989  &0.757  &1.078  &0.827    \\
                        & 336 & \textbf{0.325} & \textbf{0.366} & 0.359 &0.387 &0.339  &0.372  &1.363&0.887  &1.334  &0.872  &1.549  &0.972     \\
                        & 720 & \textbf{0.421} & \textbf{0.415} &0.433 &0.432 &0.422  &0.419  &3.379  &1.338 & 3.048 &1.328  &2.631  &1.242      \\
\midrule
\multirow{4}{*}{\rotatebox{90}{$Electricity$}} &96  & 0.193 & 0.308 &\textbf{0.183} &\textbf{0.297} &0.201  &0.317  &0.274  &0.368  &0.258  &0.357  &0.312  &0.402    \\
                        & 192 &0.201 & 0.315 & \textbf{0.195} &\textbf{0.308} &0.222  &0.334  &0.296 &0.386  &0.266 &0.368  &0.348  &0.433    \\
                        & 336 & 0.214 & 0.329 &\textbf{0.212} &\textbf{0.313} &0.231 &0.338 &0.300  &0.394  &0.280 &0.380  &0.350  & 0.433    \\
                        & 720 & 0.246 & 0.355 &\textbf{0.231} &\textbf{0.343} &0.254  &0.361  &0.373  &0.439 &0.283  &0.376  &0.340  &0.420     \\
\midrule
\multirow{4}{*}{\rotatebox{90}{$Exchange$}} &96  & 0.148 & 0.278 &\textbf{0.139} &\textbf{0.276} &0.197  &0.323  &0.847  &0.752  &0.968  &0.812  &1.065  &0.829    \\
                        & 192 & 0.271 & 0.380 &\textbf{0.256} &\textbf{0.369} &0.300  &0.369  &1.204   &0.895 &1.040  &0.851  &1.188  & 0.906   \\
                        & 336 & 0.460 & 0.500 &\textbf{0.426} &\textbf{0.464} &0.509  &0.524  &1.672  &1.036  &1.659  &1.081  &1.357  &0.976     \\
                        & 720 & 1.195 & 0.841 &\textbf{1.090} &\textbf{0.800} &1.447  &0.941  &2.478  &1.310  &1.941  &1.127  &1.510  &1.016     \\
\midrule
\multirow{4}{*}{\rotatebox{90}{$Traffic$}} &96  &0.587& 0.366 &\textbf{0.562} &\textbf{0.349} &0.613  &0.388  &0.719  &0.391  &0.684  &0.384  &0.732  &0.423    \\
                        & 192 & 0.604 & 0.373 &\textbf{0.562} &\textbf{0.346} &0.616&0.382  &0.696 &0.379  &0.685  &0.390  &0.733  &0.420    \\
                        & 336 & 0.621 & 0.383 &\textbf{0.570} &\textbf{0.323} &0.622  &0.337  &0.777  &0.420  &0.733  &0.408  &0.742  &0.420     \\
                        & 720 & 0.626 & 0.382 &\textbf{0.596} &\textbf{0.368} &0.660  &0.408  &0.864  &0.472  &0.717  &0.396  &0.755  &0.423     \\
\midrule
\multirow{4}{*}{\rotatebox{90}{$Weather$}} & 96 & \textbf{0.217} & \textbf{0.296} &0.227  &0.304  &0.266  &0.336  &0.300  &0.384  &0.458  &0.490  &0.689  &0.596    \\
                        & 192 & \textbf{0.276} & \textbf{0.336} &0.295  &0.363  &0.307  &0.367  &0.598  &0.544  &0.658  &0.589  &0.752  &0.638    \\
                        & 336 &\textbf{0.339} &\textbf{0.380} & 0.381  &0.416  &0.359  &0.395  &0.578  &0.523  &0.797  &0.652  &0.639  &0.596    \\
                        & 720 &\textbf{0.403} & \textbf{0.428} &0.424  &0.434  &0.419  &0.428  &1.059  &0.741  &0.869  &0.675  &1.130  &0.792    \\
\midrule
\multirow{4}{*}{\rotatebox{90}{$ILI$}} & 24 & 3.228 & 1.260 &\textbf{2.203}  &\textbf{0.963}  &3.483 &1.287  &5.764  &1.677  &4.480  &1.444  &4.400 &1.382    \\
                        & 36 & 2.679 & 1.080 &\textbf{2.272}  &\textbf{0.976}  &3.103  &1.148  &4.755  &1.467  &4.799  &1.467  &4.783  &1.448    \\
                        & 48 & 2.622 & 1.078 &\textbf{2.209}  &\textbf{0.981}  &2.669  &1.085  &4.763  &1.469  &4.800  &1.468  &4.832  &1.465    \\
                        & 60 & 2.854 & 1.157 &\textbf{2.545}  &\textbf{1.061}  &2.770  &1.125 &5.264  &1.564  &5.278  &1.560  &4.882  &1.483    \\
\bottomrule
\end{tabular}
\label{tab:multi-benchmarks}
}
% \end{adjustwidth}
\end{footnotesize}
\end{table*}
%}

==> tables/tab_benchmark_s_large.tex <==

\begin{table*}[t]
% \begin{adjustwidth}{-1.5in}{-1in}
\centering
\begin{small}
\caption{Univariate long-term series forecasting results on six datasets with input length $I=96$ and prediction length $O \in \{96,192,336,720\}$. A lower MSE indicates better performance.}
\scalebox{0.85}{
\begin{tabular}{c|c|cccccccccccccc}
\toprule
\multicolumn{2}{c|}{Methods}&\multicolumn{2}{c|}{FEDformer-f}&\multicolumn{2}{c|}{FEDformer-w}&\multicolumn{2}{c|}{Autoformer}&\multicolumn{2}{c|}{Informer}&\multicolumn{2}{c|}{LogTrans}&\multicolumn{2}{c}{Reformer}\\
\midrule
\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE\\
\midrule
\multirow{4}{*}{\rotatebox{90}{$ETTm2$}} 
& 96 & 0.072 & 0.206 &\textbf{0.063} &\textbf{0.189} & 0.065 & 0.189 & 0.088 & 0.225 & 0.075 & 0.208 & 0.076  &0.214   \\
& 192 & \textbf{0.102} & \textbf{0.245} &0.110 &0.252 & 0.118 & 0.256 & 0.132 &0.283 & 0.129 &0.275  & 0.132  & 0.290   \\
& 336 & \textbf{0.130} & \textbf{0.279} &0.147 &0.301 & 0.154 & 0.305  &0.180 &0.336 & 0.154 &0.302  & 0.160  & 0.312    \\
& 720 & \textbf{0.178} & \textbf{0.325} &0.219 &0.368 & 0.182 &0.335  &0.300  &0.435 & 0.160 &0.321  & 0.168  &0.335     \\
\midrule
\multirow{4}{*}{\rotatebox{90}{$Electricity$}} 
& 96  & \textbf{0.253} & \textbf{0.370} &0.262 &0.378  &0.341 &0.438 & 0.484& 0.538 &0.288& 0.393& 0.274 & 0.379 &  \\
& 192 & \textbf{0.282} & \textbf{0.386} &0.316 &0.410 &0.345 &0.428 & 0.557& 0.558 &0.432 & 0.483 & 0.304 &0.402 &  \\
& 336 & \textbf{0.346} & \textbf{0.431} &0.361 &0.445 &0.406 &0.470 & 0.636& 0.613 &0.430 &0.483 & 0.370 &0.448 & \\
& 720 & \textbf{0.422} & \textbf{0.484} &0.448 &0.501 &0.565 &0.581 & 0.819& 0.682 &0.491 &0.531 & 0.460 &0.511 &  \\
\midrule

\multirow{4}{*}{\rotatebox{90}{$Exchange$}} 
&96  & 0.154 & 0.304 &\textbf{0.131} &\textbf{0.284} & 0.241 & 0.387  & 0.591  &0.615  &0.237 &0.377  &0.298  &0.444    \\
& 192 & 0.286 & 0.420 &\textbf{0.277} &\textbf{0.420} &0.300  &0.369  &1.183   &0.912 &0.738  &0.619  &0.777  & 0.719   \\
& 336 & 0.511 & 0.555 &\textbf{0.426} &\textbf{0.511} &0.509  &0.524  &1.367  &0.984  &2.018  &1.070  &1.832  &1.128     \\
& 720 & 1.301 & 0.879 &\textbf{1.162} &\textbf{0.832} &1.260  &0.867  &1.872  &1.072  &2.405  &1.175  &1.203  &0.956     \\
\midrule
\multirow{4}{*}{\rotatebox{90}{$Traffic$}} 
&96  & 0.207 & 0.312 &\textbf{0.170} &\textbf{0.263}  &0.246 &0.346 & 0.257 & 0.353 &0.226 &0.317 &  0.313 & 0.383\\
& 192 & 0.205 & 0.312 &\textbf{0.173} &\textbf{0.265} &0.266 &0.370 & 0.299 & 0.376 &0.314 &0.408 & 0.386 & 0.453\\
& 336 & 0.219 & 0.323 &\textbf{0.178} &\textbf{0.266} &0.263 &0.371 & 0.312 & 0.387 &0.387 &0.453 & 0.423 & 0.468\\
& 720 & 0.244 & 0.344 &\textbf{0.187} &\textbf{0.286} &0.269 &0.372 & 0.366 & 0.436 &0.491 &0.437 & 0.378 & 0.433\\
\midrule
\multirow{4}{*}{\rotatebox{90}{$Weather$}}
& 96  & 0.0062 & 0.062 & \textbf{0.0035} & \textbf{0.046} & 0.011 &0.081 & 0.0038 & 0.044 & 0.0046 &0.052 & 0.012 & 0.087 \\
& 192 & 0.0060& 0.062&\textbf{0.0054} &\textbf{0.059} &0.0075 &0.067 & 0.0023 & 0.040 &0.0056 & 0.060 & 0.0098 & 0.079  \\
& 336 & \textbf{0.0041} & \textbf{0.050} &0.008 &0.072 &0.0063 &0.062 & 0.0041 & 0.049 &0.0060 &0.054& 0.0050 & 0.059 \\
& 720 & 0.0055 & 0.059 &0.015 &0.091 &0.0085 &0.070 & 0.0031 & 0.042 &0.0071 &0.063& \textbf{0.0041} & \textbf{0.049} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{$ILI$}} 
& 24 & 0.708 & 0.627 &\textbf{0.693} &\textbf{0.629} &0.948 &0.732 & 5.282 &2.050 &3.607 & 1.662 & 3.838 & 1.720  \\
& 36 & 0.584 & 0.617 &\textbf{0.554} &\textbf{0.604} &0.634 &0.650 & 4.554 &1.916 &2.407 & 1.363 & 2.934 & 1.520 \\
& 48 & 0.717 & 0.697 &\textbf{0.699} &\textbf{0.696} &0.791 &0.752 & 4.273 &1.846 &3.106 & 1.575 & 3.754 & 1.749\\
& 60 & 0.855 & 0.774 &\textbf{0.828} &\textbf{0.770} &0.874 &0.797 & 5.214 &2.057 &3.698 & 1.733 & 4.162 & 1.847\\
\bottomrule
\end{tabular}
}
\label{tab:uni-benchmarks-large}
% \end{adjustwidth}
\end{small}
\end{table*}


==> tables/tab_benchmark_s_small.tex <==

\begin{table*}[t]
\centering
% \begin{adjustwidth}{-1.5in}{-1in}
\begin{footnotesize}
\caption{Univariate long-term series forecasting results on two typical datasets with input length $I=96$ and prediction length $O \in \{96,192,336,720\}$. A lower MSE indicates better performance.}
\scalebox{0.85}{
\begin{tabular}{c|c|cccccccccccccccc}
\toprule
\multicolumn{2}{c|}{Methods}&\multicolumn{2}{c|}{FEDformer-f}&\multicolumn{2}{c|}{FEDformer-w}&\multicolumn{2}{c|}{Autoformer}&\multicolumn{2}{c|}{Informer}&\multicolumn{2}{c|}{LogTrans}&\multicolumn{2}{c}{Reformer}\\
\midrule
\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE\\
\midrule
\multirow{4}{*}{\rotatebox{90}{$ETTm2$}} 
& 96 & 0.072 & 0.206 & \textbf{0.063} & \textbf{0.189} & 0.065 & 0.189 & 0.088 & 0.225 & 0.082 & 0.217 & 0.131  &0.288    \\
& 192 & \textbf{0.102} & \textbf{0.245} &0.110 &0.252 & 0.118 & 0.256 & 0.132 &  0.283 & 0.133  &0.284  &0.186  &0.354    \\
& 336 & \textbf{0.130} & \textbf{0.279} &0.147 &0.301 & 0.154 & 0.305  &0.180 &0.336  & 0.210  &0.361  &0.220  &0.381     \\
& 720 & \textbf{0.178} & \textbf{0.325} &0.219 &0.368 & 0.182 &0.335  &0.300  &0.435 & 0.268 &0.407  &0.267  &0.430      \\
\midrule

% \multirow{5}{*}{\rotatebox{90}{$Electricity$}} 
% &96  & 0.154 & 0.304 & & & 0.241 & 0.387  & 0.591  &0.615  &0.279 &0.441  &1.327  &0.944    \\
% & 192 & 0.286 & 0.420 & & &0.300  &0.369  &1.183   &0.912 &1.950  &1.048  &1.258  & 0.924   \\
% & 336 & 0.511 & 0.555 & & &0.509  &0.524  &1.367  &0.984  &2.438  &1.262  &2.179  &1.296     \\
% & 720 & 1.301 & 0.879 & & &1.447  &0.941  &1.872  &1.072  &2.010  &1.247  &1.280  &0.953     \\

\multirow{4}{*}{\rotatebox{90}{$Exchange$}} 
&96  & 0.154 & 0.304 &\textbf{0.131} &\textbf{0.284} & 0.241 & 0.387  & 0.591  &0.615  &0.279 &0.441  &1.327  &0.944    \\
& 192 & 0.286 & 0.420 &\textbf{0.277} &\textbf{0.420} &0.300  &0.369  &1.183   &0.912 &1.950  &1.048  &1.258  & 0.924   \\
& 336 & 0.511 & 0.555 &\textbf{0.426} &\textbf{0.511} &0.509  &0.524  &1.367  &0.984  &2.438  &1.262  &2.179  &1.296     \\
& 720 & 1.301 & 0.879 &\textbf{1.162} &\textbf{0.832} &1.260  &0.867  &1.872  &1.072  &2.010  &1.247  &1.280  &0.953     \\
\bottomrule
\end{tabular}
\label{tab:uni-benchmarks-small}
}
% \end{adjustwidth}
\end{footnotesize}
\end{table*}


==> tables/tab_length.tex <==

\begin{table*}[t]
% \begin{adjustwidth}{-1.5in}{-1in}
\begin{small}
\begin{tabular}{c|c|cccccccc}
\toprule
\multicolumn{2}{c|}{Methods}&\multicolumn{2}{c|}{Fedform-f}&\multicolumn{2}{c|}{Autoformer}&\multicolumn{2}{c|}{Informer}. \\%&\multicolumn{2}{c|}{}&\\
\midrule
\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE \\%& MSE  & MAE \\
\midrule
\multirow{5}{*}{{96}} 
& 336  & 0.326 & 0.367 & 0.339 & 0.372 & 0.481 & 0.472\\
& 720  & 0.418 & 0.414 & 0.422 & 0.419 & 0.822 & 0.559\\
& 1440 & 0.475 & 0.502 & 0.555 & 0.496 & 0.715 & 0.586\\
\midrule
\multirow{5}{*}{{192}} 
% & 96  & 0.239 & 0.315 & 0.273 & 0.345 & 0.560\\
% & 192 & 0.283 & 0.341 & 0.364 & 0.391 & 1.331\\
& 336 & 0.331 & 0.375 & 0.355 & 0.392 & 0.404 & 0.425\\
& 720 & 0.422 & 0.428 & 0.429 & 0.430 & 1.148 & 0.654\\ 
& 1440& 0.482 & 0.472 & 0.503 & 0.484 & 0.732 & 0.602\\
% & 672 & 0.606 & & 0.528 & & 0.544 & & 0.501\\
% & 720 & 0.658 & 0.548 & \textbf{0.543} & 0.517 & 0.558 & \textbf{0.507} & 0.543 & 0.490\\
\midrule
\multirow{5}{*}{{336}} 
% & 96 & 0.255 & 0.339 & 0.259  & 0.337& \textbf{0.216} &\textbf{0.297} & 0.203 & 0.287      \\
% & 192 & 0.304 & 0.366 & 0.415 & 0.438 & \\
& 336 & 0.339 & 0.388 & 0.361 & 0.406 & 0.417 & 0.434\\
& 720 & 0.418 & 0.431 & 0.425 & 0.440 & 0.631 & 0.528\\
& 1440& 0.467 & 0.471 & 0.574 & 0.534 & 1.133 & 0.691\\
% \midrule
% \multirow{5}{*}{{720}} 
% % & 96 & 0.255 & 0.339 & 0.259  & 0.337& \textbf{0.216} &\textbf{0.297} & 0.203 & 0.287      \\
% % & 192 & \\
% & 336 & 0.449 & 0.484 & 0.496 & 0.497\\
% & 720 & 0.496 & 0.531 & 0.600 & 0.552\\
% & 1440 & 0.437 & 0.472& 0.660 & 0.581\\
\bottomrule
\end{tabular}
\caption{Sequence length.}
\label{tab:length}
% \end{adjustwidth}
\end{small}
\end{table*}

==> tables/tab_modes.tex <==

\begin{table*}[t]
% \begin{adjustwidth}{-1.5in}{-1in}
\begin{tabular}{c|c|cccccccccccc}
\toprule
\multicolumn{2}{c|}{Methods}&\multicolumn{2}{c|}{Modes=4}&\multicolumn{2}{c|}{Modes=8}&\multicolumn{2}{c|}{Modes=16}&\multicolumn{2}{c|}{Modes=32}&\multicolumn{2}{c|}{Dynamic}&\\
\midrule

% \multirow{2}{*}{Detail}
% & Self-att & \multicolumn{2}{c|}{AutoCorrelation} & \multicolumn{2}{c|}{FNO (Eq. \ref{func:FNO-self})} & \multicolumn{2}{c|}{AutoCorrelation} & \multicolumn{2}{c|}{FNO (Eq. \ref{func:FNO-self})}\\
% & Corss-att & \multicolumn{2}{c|}{AutoCorrelation} & \multicolumn{2}{c|}{AutoCorrelation} & \multicolumn{2}{c|}{FNO (Eq. \ref{func:FNO-Corss})} & \multicolumn{2}{c|}{FNO (Eq. \ref{func:FNO-Corss})}\\
% \midrule

\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE & MSE  & MAE \\
\midrule
\multirow{4}{*}{\rotatebox{90}{ETTm1}} 
& 192 & 0.628 & 0.526 & \textbf{0.417} & \textbf{0.442} & \textbf{0.556} & \textbf{0.499} & \textbf{0.426} & \textbf{0.441}\\
& 336 & 0.728 & 0.567 & \textbf{0.480} & \textbf{0.477} & \textbf{0.541} & \textbf{0.498} & \textbf{0.445} & \textbf{0.459}\\
& 720 & 0.658 & 0.548 & \textbf{0.543} & \textbf{0.517} & \textbf{0.558} & \textbf{0.507} & \textbf{0.543} & \textbf{0.490}\\
% \midrule
\midrule

\multirow{3}{*}{\rotatebox{90}{ETTm2}} 
& 192 & 0.268 & 0.327 & 0.265& 0.325 & 0.266 & 0.326 & 0.267 & 0.328 & 0.269 & 0.328\\

& 336 & 0.332 & 0.370 & 0.332 & 0.370 & 0.329 & 0.367 & 0.326 & 0.364 & \textbf{0.325} & \textbf{0.366}\\
& 720 & 0.443 & 0.433 & 0.443 & 0.433 & 0.434 & 0.443 & 0.437 & 0.428 & \textbf{0.421} & \textbf{0.415}\\

% \midrule
% \multicolumn{2}{c|}{Count} & 1 & 1 & 5 & 5 & 6 & 6 & 8 & 8\\
\bottomrule
\end{tabular}
\caption{Modes: multivariate long sequence time-series forecasting results on six datasets.}
\label{tab:modes}
% \end{adjustwidth}
\end{table*}
